Zorro: A Model Agnostic System to Price Consumer Data

Personal data is essential in showing users targeted ads - the economic backbone of the web. Still, there are major inefficiencies in how data is transacted online: (1) users don't decide what information is released nor get paid for this privacy loss; (2) algorithmic advertisers are stuck in inefficient long-term contracts where they purchase user data without knowing the value it provides. This paper proposes a system, Zorro, which aims to rectify aforementioned two problems. As the main contribution, we provide a natural, 'absolute' definition of 'Value of Data' (VoD) - for any quantity of interest, it is the delta between an individual's value and population mean. The challenge remains how to operationalize this definition, independently of a buyer's model for VoD. We propose a model-agnostic solution, relying on matrix estimation, and use it to estimate click-through-rate (CTR), as an example. Regarding (2), Zorro empowers advertisers to measure value of user data on a query-by-query basis and based only on the increase in accuracy it provides in estimating CTR. In contrast advertisers currently engage in inefficient long-term data contracts with third party data sellers. We highlight two results on a large ad-click dataset: (i) our system has R^2=0.58, in line with best-in-class results for related problems (e.g. content recommendation). Crucially, our system is model-agnostic - we estimate CTR without accessing an advertiser's proprietary models, a required property of any such pricing system;(ii) our experiments show selling user data has incremental value ranging from 30%-69% depending on ad category. Roughly, this translates to at least USD 16 Billion loss in value for advertisers if user data is not provided. Regarding (1), in addition to allowing users to get paid for data sharing, we extend our mathematical framework to when users provide explicit intent.

==> content/experiments_old.tex <==
\section{Experiments}\label{sec:experiments}

This section is organized into four sets of experiments: 
\begin{enumerate}
	\item \textbf{Matrix Estimation.} How accurately matrix estimation is able to estimate the underlying CTR.
	\item \textbf{VoD.} The amount of variation in VoD for user data depending on an advertiser's category
	\item \textbf{Ad Data Collection.} How accurately we identify and categorize ads.
	\item \textbf{User Data Protection.} Whether we can reliably prevent user data from being ``leaked" to advertisers
\end{enumerate}

\subsection{Matrix Estimation Experiments}\label{sec:ME_experiments}

\noindent \textbf{Matrix Estimation Algorithms Applied.} We focus on two well-studied matrix estimation algorithms, Alternating Least Squares (ALS) and Singular Value Thresholding (SVT). See cf.~[\ref{}] for a detailed description of these algorithms and theoretical guarantees of convergence and quality of the final estimate. For ALS, we rely on a standard PySpark implementation (cf.~[\ref{}]) and for SVT, we use the NumPy package (cf.~[\ref{}]) to perform the singular value decomposition. Lastly, we implement a hybrid two-step algorithm that first does SVT on the observation matrix and uses the outputted matrix as a ``warm start" for ALS. 

\vspace{2mm}

\noindent \textbf{Metric Used to Measure Accuracy.} We measure quality of performance using $R^2$. 

\subsubsection{Avazu Dataset}\label{sec:avazu_dataset}

\noindent \textbf{Description of Dataset Used.} We test our system on the Avito Context Ad Clicks dataset. To the best of our knowledge, it is the largest and most comprehensive publicly available ad click dataset. It can be found on Kaggle (cf.~[\ref{}]).  Avito is the largest online marketplace in Russia with 70 million unique monthly visitors. Another reason we use this dataset is that its focus is contextual ads (i.e. banner ads), which is also the focus of our work.

There are $190,157,735$ context ad views in the dataset, out of which $1,146,289$ led to clicks. For each view, the dataset includes metadata about the user (e.g. geographic location, parameters of the search) and the ad itself (e.g. category of the ad, historical CTR), along with whether the view led to a click or not.

\vspace{2mm}

\noindent \textbf{Grouping Users \& Advertisers.} We group users by their geographical location (there are {\color{red} xxx} unique location ids) and ads by their category (there are {\color{red} xxx} unique category ids). We choose location as it is a standard feature used in CTR estimation, and related tasks. However, many other user features can and should be incorporated in practice. Indeed, our experiments are meant to showcase accurate CTR estimation is possible by simple groupings of users. Similarly, in practice advertisers are commonly grouped by category (see Section \ref{sec:ad_categorization}) and hence we do so as well. 

\vspace{2mm}

\noindent \textbf{Data Preprocessing.} In Figure \ref{fig:ME_data_quality_1}, we plot a histogram of empirical CTR for each user in the Avazu dataset (on a log scale). We see a large number of user CTRs that are unreasonably high (e.g. there is a spike at $1.0$). Indeed, a known issue in such datasets is ``click-bots" which are programs that automatically click on ads to increase revenue in a fraudulent manner. That is why we filter out all users beyond a certain threshold, specifically $0.02$. We do so because according to historical Google AdWords data, ``human" CTR for different advertiser categories ranges between $0.0035$ and $0.02$. (cf.~[\ref{}]). 

This choice of threshold is justified empirically through Figure \ref{fig:ME_data_quality_2}. We create a matrix of users and advertisers (grouped according to location and category respectively), take its singular value decomposition, and then plot the singular values of this matrix for different thresholds. If we don't threshold (i.e. keep the threshold at $1.0$), then the spectrum decays very gradually. However, as we decrease the threshold, the spectrum decays progressively quicker, and the low-rank structure we expect to see emerges (see Section \ref{sec:computing_value_of_data}). The optimal threshold is approximately at $0.02$, and at this threshold, we still retain $81\%$ of the original data.

\subsubsection{Matrix Estimation Results}\label{sec:ME_experiments_results}

\noindent \textbf{Hyper-parameter Selection.} For both ALS and SVT, there is one major hyper-parameter to choose, the number of singular values to keep. From Figure \ref{fig:ME_data_quality_2}, we see that the top two singular values contain most of the ``signal" and hence we choose to keep two singular values. This is further justified through cross-validation. In PySpark's implementation of ALS, a regularization parameter must also be chosen, which we set to be $0.01$, again using cross-validation.

\vspace{2mm}

\noindent \textbf{CTR Estimation via Matrix Estimation Experiments.} Figures \ref{fig:ME_percent_matrix_filled_1}-\ref{fig:ME_percent_holdout_3} show how the quality of matrix estimation changes as we vary: (1) the percentage of entries observed; (2) the number of data points used; (3) percentage of data used for out-of-sample testing. 

For Figures \ref{fig:ME_percent_matrix_filled_1}-\ref{fig:ME_data_points_3}, we keep the percentage of data withheld for out-of-sample testing to be fixed at $20\%$. We see that $R^2$ performance of the various algorithms improves steadily as the fraction of data observed and the number of data points increases (with ALS outperforming SVT). However, this improvement levels off after approximately $40\%$ of the data is observed and $50$ million data points are used. This indicates two takeaways with regards to accurate CTR estimation: (1) some amount of grouping of users and advertisers is an important pre-processing to ensure the resulting matrix is not too sparse; (2) our system needs to collect approximately on the order of tens of millions of user data to apply matrix estimation effectively.

Additionally, from Figures \ref{fig:ME_percent_holdout_1}-\ref{fig:ME_percent_holdout_3}, we see $R^2$ improves as we decrease the percentage of data withheld for out-of-sample testing, as expected.

\vspace{2mm}

\noindent \textbf{Signal vs. Noise Thresholding via Matrix Estimation.} From Section \ref{sec:computing_value_of_data}, we know that matrix estimation should help uncover the underlying mean of the CTR matrix, $\bM$, while reducing the noise as long as the underlying matrix is low-rank (which we verified through Figure \ref{fig:ME_data_quality_2}). In particular for the Avazu dataset, we expect that the average CTR per advertiser category should remain approximately the same both before and after applying matrix estimation
\footnote{There are a large number of user location id's ({\color{red} xxx} of them). Thus the pre-$\text{ME}$ estimate of CTR per advertiser category should be relatively stable.}. 
However, the variance in CTR per advertiser category should drop significantly. 

We recall the notation used in Section \ref{sec:computing_value_of_data}. Let 
\[
\hmupre^j := \frac{1}{\text{\# observed}}\sum_{i=1}^m \bX_{ij} \mathbbm{1}(\bX_{ij} \neq ?), \ \ \ \hmupost^j := \frac{1}{m}\sum_{i=1}^m \hM_{ij}.
\]
In words, $\hmupre^j, \hmupost^j$ are the pre-$\text{ME}$ and post-$\text{ME}$ empirical average CTRs for each advertiser category $j$ in the Avazu dataset. Let,
\begin{align*}
\hvarpre^j &:= \frac{1}{\text{\# observed}} \sum_{i=1}^m  (\bX_{ij} \mathbbm{1}(\bX_{ij} \neq ?) - \hmupre^j)^2, \\
\hvarpost^j &:= \frac{1}{m}\sum_{i=1}^m (\hM_{ij} - \hmupost^j)^2.
\end{align*}
In words, $\hvarpre^j, \hvarpost^j$ are the pre-$\text{ME}$ and post-$\text{ME}$ empirical variance in CTR for each advertiser category $j$ in the Avazu dataset.

In Figures \ref{fig:ME_signal_vs_noise_1}-\ref{fig:ME_signal_vs_noise_3}, we plot the normalized differences in mean and variance per advertiser category
\footnote{We normalize by $\hmupre^j$ to ensure $\hmudiff$ can be appropriately compared between categories. For example, a $0.1$ difference is significant if the underlying average CTR is $0.01$, but not as much if it is $0.5$. Same reasoning applies for $\hvardiff$.},
\[
\hmudiff := \frac{1}{\hmupre^j}|\hmupre^j -  \hmupost^j|, \ \ \ \hvardiff := \frac{1}{(\hmupre^j)^2}|\hvarpre^j - \hvarpost^j|.
\]
We see from Figure \ref{fig:ME_signal_vs_noise_3} that $\hmudiff$ is of the order {\color{red} $10\%-80\%$}, while $\hvardiff$ is of the order {\color{red} $800\%- 1200\%$}. Thus as desired, $\hmudiff$ is three orders of magnitude smaller than $\hvardiff$, indicating that matrix estimation does indeed effectively retain signal and threshold out noise.

\vspace{2mm}

\noindent \textbf{Summary.} In summary, ALS outperforms SVT (the two-step procedure of applying SVT and then ALS gives comparable performance). The best $R^2$ achieved is {\color{red} $0.6$}; This is in-line with or better than state-of-the-art $R^2$ performance for well-studied datasets such as Movielens, which have performance in the range of {\color{red} $0.35-0.45$ (cf.~[\ref{}])}. Further, our experiments show that matrix estimation does effectively retain signal and threshold out noise.

Thus matrix estimation (specifically, ALS) can be used as an accurate, model-agnostic method to do CTR estimation as long as Zorro has access to sufficient amount of user data, and careful grouping of users and advertiser is done.

\begin{figure}%
\centering

\subfigure[]{%
\label{fig:ME_data_quality_1}%
\includegraphics[width=0.5\linewidth,height=2.5cm]{figures/2_data_quality/2a_hist.png}}%
\hfill
\subfigure[]{%
\label{fig:ME_data_quality_2}%
\includegraphics[width=0.5\linewidth,height=2.5cm]{figures/2_data_quality/2b_rank_threshold.png}}%
\vspace{-3mm}
\caption{Figure \ref{fig:ME_data_quality_1} - Histogram of CTR for different users
%; we can visually see that many spurious outliers exist (e.g. spike at CTR of 1.0)
. Figure \ref{fig:ME_data_quality_2} - Plot of Singular Values at different CTR thresholds and percentage of data retained.}

\vspace{1mm}

\subfigure[]{%
\label{fig:ME_percent_matrix_filled_1}%
\includegraphics[width=0.33\linewidth,height=2.5cm]{figures/3_percent_matrix/3a_svt_percent_matrix.png}}%
\hfill
\subfigure[]{%
\label{fig:ME_percent_matrix_filled_2}%
\includegraphics[width=0.33\linewidth,height=2.5cm]{figures/3_percent_matrix/3b_als_percent_matrix.png}}%
\hfill
\subfigure[]{%
\label{fig:ME_percent_matrix_filled_3}%
\includegraphics[width=0.33\linewidth,height=2.5cm]{figures/3_percent_matrix/3c_svt_als_percent_matrix.png}}%
\vspace{-3mm}
\caption{$R^2$ vs. \% Matrix Filled for SVT, ALS and SVT +  ALS. In-Sample and Out-of-Sample performance plotted.}

\vspace{1mm}

\subfigure[]{%
\label{fig:ME_data_points_1}%
\includegraphics[width=0.33\linewidth,height=2.5cm]{figures/4_data_points/4a_svt_data_points.png}}%
\hfill
\subfigure[]{%
\label{fig:ME_data_points_2}%
\includegraphics[width=0.33\linewidth,height=2.5cm]{figures/4_data_points/4b_als_data_points.png}}%
\hfill
\subfigure[]{%
\label{fig:ME_data_points_3}%
\includegraphics[width=0.33\linewidth,height=2.5cm]{figures/4_data_points/4c_svt_als_data_points.png}}%
\vspace{-3mm}
\caption{$R^2$ vs. \# Data Points used for SVT, ALS and SVT +  ALS. In-Sample and Out-of-Sample performance plotted.}

\vspace{1mm}

\subfigure[]{%
\label{fig:ME_percent_holdout_1}%
\includegraphics[width=0.33\linewidth,height=2.5cm]{figures/5_percent_holdout/5a_svt_percent_holdout.png}}%
\hfill
\subfigure[]{%
\label{fig:ME_percent_holdout_2}%
\includegraphics[width=0.33\linewidth,height=2.5cm]{figures/5_percent_holdout/5b_als_percent_holdout.png}}%
\hfill
\subfigure[]{%
\label{fig:ME_percent_holdout_3}%
\includegraphics[width=0.33\linewidth,height=2.5cm]{figures/5_percent_holdout/5c_svt_als_percent_holdout.png}}%
\vspace{-3mm}
\caption{$R^2$ vs. \% Out-of-Sample for SVT, ALS and SVT +  ALS. In-Sample and Out-of-Sample performance plotted.}

\vspace{1mm}

\subfigure[]{%
\label{fig:ME_signal_vs_noise_1}%
\includegraphics[width=0.33\linewidth,height=2.5cm]{figures/6_vod_plots/6a_mean.png}}%
\hfill
\subfigure[]{%
\label{fig:ME_signal_vs_noise_2}%
\includegraphics[width=0.33\linewidth,height=2.5cm]{figures/6_vod_plots/6b_var.png}}%
\hfill
\subfigure[]{%
\label{fig:ME_signal_vs_noise_3}%
\includegraphics[width=0.33\linewidth,height=2.5cm]{figures/6_vod_plots/6c_log_percentage.png}}%
\vspace{-3mm}
\caption{Figures \ref{fig:ME_signal_vs_noise_1}-\ref{fig:ME_signal_vs_noise_2} - Plot of difference in empirical mean and variance per category pre- and post-ME respectively. Figure \ref{fig:ME_signal_vs_noise_3} - \% Difference in $\hat{\mu}$ and $\widehat{\text{var}}$ per category plotted on log scale.}

\end{figure}

%$|\hat{\mu}_{\text{pre}} - \hat{\mu}_{\text{post}}|$

\subsection{Value of Data Experiments}\label{sec:VoD_experiments}

An important question to ask is if with respect to Definition \ref{def:estimated_VoD_definition} of VoD, whether an advertiser find value in a user's personal data? 
Intuitively, if the CTR distribution for a particular advertiser category is tightly concentrated around its mean, then acquiring user data is not as important for that advertiser (as there is not much variation in CTR across users). In contrast, if the CTR distribution for an advertiser category is diffuse, then advertisers are incentivized to acquire personal user data as it helps them identify which segment of the distribution a user lies in. 

\vspace{2mm}

\noindent \textbf{Large Variation in VoD Across Advertiser Categories.} We plot the distribution of CTR per category using a Box-and-Whisker's plot in Figure \ref{fig:VoD_variation_1}, and see instances of both cases above. For example, advertisers in Category 18 have relatively lower VoD as the CTR distribution is tightly concentrated, while advertisers in Category 4 have quite a large VoD as the CTR distribution is quite diffuse. Thus we can visually tell that advertiser's do indeed have a different VoD depending on their category, giving credence to Definition \ref{def:estimated_VoD_definition}. 

We can summarize these visual findings through the following quantity,
\[
\hVoDUser_j := \frac{1}{\hmupre^j}\bigg(\frac{1}{m}\sum_{i =1}^m \hVoD \bigg).
\]
In words, $\hVoDUser_j$ is the average VoD Advertiser $j$ experiences per user
\footnote{Again, like in Section \ref{sec:ME_experiments_results}, we normalize by $\hmupre^j$ to ensure we can appropriately compare between categories.}. 
In Figure \ref{fig:VoD_variation_2}, we plot $\hVoDUser_j$ for the various Avazu categories. We see that $\hVoDUser_j$ ranges from {\color{red} 25\% to 65\%} depending on advertiser category, indicating that there is large variation in VoD depending on which category an advertiser belongs to.

\vspace{2mm}

\noindent \textbf{Query-by-Query Estimation of VoD.} It is important to highlight that in our proposed system, Advertiser $j$ can compute the VoD on a query-by-query basis. In other words, each time User $i$ loads a webpage, Advertiser $j$ can compute $\hVoD$. This is contrast with how advertiser's and third-party data providers engage currently, where advertisers pay based on long-term contracts or a coarse metric such as number of API calls made.

%Depending on If the distribution of CTR for Advertiser $j$'s category is tightly concentrated around the mean (i.e. $\hVoDUser_j$ is small), then as per the dynamics laid out in Section \ref{sec:dsp_zorro_interface}, Advertiser $j$ will on average pay relatively less for User $i$'s data. 

\vspace{2mm}

\noindent \textbf{Estimating Dollar Value of VoD.} \Anish{What should we put here? We can't map category IDs to actual categories}

\begin{figure}%
\centering
\subfigure[]{%
\label{fig:VoD_variation_1}%
\includegraphics[width=0.5\linewidth,height=3cm]{figures/7_vod_plots_2/7a_post_me_box.png}}%
\hfill
\subfigure[]{%
\label{fig:VoD_variation_2}%
\includegraphics[width=0.5\linewidth,height=3cm]{figures/7_vod_plots_2/7b_percent_info.png}}%
\vspace{-3mm}
\caption{Figure \ref{fig:VoD_variation_1} - Box and Whisker's plot of CTR distribution per category. Figure \ref{fig:VoD_variation_2} - Plot of normalized average $\widehat{\text{VoD}}$ per category.}
\end{figure}


\subsection{Online Ad Experiments}\label{sec:ad_experiments}

In this section, we focus on testing how well we can identify and categorize online ads by tying together existing open source software packages.

%A necessary step to do CTR estimation, is to accurately identify when users have clicked on an ad. Further to effectively group advertisers, we need to categorize advertisers in a meaningful and automated way. We show how to do both ad identification and categorization by tying together existing open source software packages.

%\noindent \textbf{Definition of Ad.}  Below we describe a straightforward two-level filter system to identify ads when a user clicks on a link on a website. 
%
%\begin{enumerate}
%	\item \textbf{Filter Level 1.} We filter for hyperlinks on a website that redirect to a url external to the website itself. 
%	\item \textbf{Filter Level 2.} We parse the redirect url to check for substrings that are almost always present when the external link redirects to ads hosted by third-party servers (e.g. AdChoices, Outbrain). We do this by filtering the redirect url using the industry standard Easylist filter list (cf.~[\ref{}]), which is a set of rules designed by AdBlock (cf.~[\ref{}]) to identify ads. 
%\end{enumerate}
%
%In Section \ref{sec:ad_experiments}, we show that this simple system effectively identifies whether an external hyperlink is an ad (True Positive and True Negative rate of {\color{red} $83\%$ and $97\%$} respectively). 

\subsubsection{Online Ad Identification} \subsubsection{Classification Method}

\noindent \textbf{Overview of Ad Identification Module.} Recall from Section \ref{sec:ad_identification} that the main filter we use on the redirect url is EasyList, the same filter set used by AdBlock. In addition, we manually added keywords such as “doubleclick” and “criteo” that commonly occur when a user has clicked on an ad.

\vspace{2mm}

\noindent \textbf{Overview of Ad Identification Experiment.} To evaluate this simple system, we conducted a crowdsourced experiment. The experiment consisted of iterating through Alexa’s top 500 global sites (cf.~[\ref{}]) and clicking ten unique ads on each site. Websites that are not in English or had no ads were skipped. If there were not ten unique ads on the websites landing page, then ads on different webpages under the some domain were searched for. Additionally, hyperlinks that were not ads were also clicked to test whether our system could also identify non-ads accurately. 

\vspace{2mm}

\noindent \textbf{Result of Ad Identification Experiment.} The result of the above crowdsourced experiment are shown in Table \ref{tab:AD_identification_table}. We have True Positive rate of $83\%$ and a True Negative Rate of $97\%$, indicating that our system can reliably identify whether a hyperlink on a webpage is an ad or not. Additionally, a large portion of the ads we could not identify were because they did not go through an ad exchange (i.e. have a redirect url that spawned a tab in a browser). If we do not include such ads, then our True Positive rates goes up to {\color{red} xxx \%}. Such ads are the result of direct negotiations between a website and advertisers. Thus they are not of relevance to our system as they do not go through the RTB ecosystem, and third-party data is not purchased by advertisers in such instances.

\begin{table}[h!]
  \begin{center}
    \begin{tabular}{l|c|r} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
       & \textbf{True Ad} & \textbf{Not Ad}\\
%      $\alpha$ & $\beta$ & $\gamma$ \\
      \hline
      \textbf{Classified Ad} & 239 (83\%) & 49 (17\%)\\
      \textbf{Classified Not Ad} & 2 (97\%) & 68 (3\%)\\
   \end{tabular}
  \end{center}
   \caption{}
   \label{tab:AD_identification_table}
\end{table}

\subsubsection{Online Ad Categorization}

\noindent \textbf{Overview of Ad Categorization Module.} Recall from Section \ref{sec:ad_categorization} (and experimentally verified in Section \ref{sec:ME_experiments_results}) that ad categorization is an important pre-processing step to group advertiser's together to get good out-of-sample performance in CTR estimation. As detailed in Section \ref{sec:ad_categorization}, we use the industry standard IAB taxonomy to categorize advertisers. To do so, we use the open-source natural language processing software uClassify to predict a webpage's IAB category based on the text in the webpage's body. We focus on the top two Tiers of the IAB taxonomy as the categorization is sufficiently detailed. It is straightforward to extend to the bottom two tiers if required. 

\vspace{2mm}

\noindent \textbf{Overview of Ad Categorization Experiment.} Unfortunately, there do not exist good online datasets with IAB categorizations of websites that we can use to test the accuracy of our system. Thus we designed a proxy experiment using Wikipedia webpages as follows. Wikipedia provides a detailed hierarchal categorization of its own webpages (cf.~[\ref{}]). For each IAB Tier 1 category ($28$ in total), we randomly sample two Tier 2 categories within it. We then define a mapping from these IAB Tier 2 category to a near identical Wikipedia category ({\color{red} give an example}). If a close Wikipedia category was not found, we resample an IAB Tier 2 category such that a matching Wikipedia is found.

For each Wikipedia category selected, we chose up to 100 articles under that category. If there are not 100 articles for a given Wikipedia category (for many there were not), we iterated through the subcategories of that category, and randomly sampled articles from those subcategories until we reached a 100. We then ran our classifier on the text from those articles. 

\vspace{2mm}

\noindent \textbf{Result of Ad Categorization Experiment.} The results of the above  experiment are shown in Figures \ref{fig:AD_cat_1} and \ref{fig:AD_cat_2}. For Tier 1 categories, the classification accuracy was 67.36$\%$ and for Tier 2 categories, the classification accuracy was 52.75$\%$. This is consistent as correctly classifying a Tier 1 category is a necessary requirement to correctly classify Tier 2 category.

It is worth noting that these results are far better than if we random selected a category. Recall that there are 28 IAB Tier 1categories and 341 Tier 2 categories and so a random classification would give $3.6\%$ and $0.3\%$ accuracy respectively. 

Furthermore, it is likely that our system performs better than our tests indicate for the following two reasons. (1) It was often that case that articles from subcategories of the selected Wikipedia category were somewhat unrelated the further down in the Wikipedia hierarchy the subcategory was ({\color{red} give example}). (2) If an outputted IAB category was incorrect, it was still  often strongly related to the correct one. For example, articles on children’s films would be classified as family films or fantasy films. 

Considering these relatively benign sources of error, and the large number of Tier 1 and Tier 2 categories, our system reliably categorizes an advertiser to a relevant IAB category, based on the advertiser's webpage.

\begin{figure}[ht]
\centering
\includegraphics[width=0.7\linewidth,height=4cm]{figures/AD_cat_1.png}
\caption{uClassify classifier accuracy on IAB Tier 1 categories. Average accuracy is 67.36\%.}
\label{fig:AD_cat_1}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width=0.7\linewidth,height=4cm]{figures/AD_cat_2.png}
\caption{uClassify classifier accuracy on IAB Tier 2 categories. Average accuracy is 52.75\%.}
\label{fig:AD_cat_2}
\end{figure}

\subsection{User Data Protection Experiments}\label{sec:protecting_user_data}

Recall from Section \ref{sec:dsp_zorro_interface} that for our system to work, it is essential that if a user is using the Zorro system, his or her personally identifiable information (PII) is not inadvertently ``leaked" to advertisers. We begin by giving a brief overview of how advertisers track users across the web and then describe an experiment to verify that user data is indeed not leaked to an advertiser.

\vspace{2mm}

\noindent \textbf{Tracking Techniques.} As users surf the web, advertisers track users through three main methods (cf.~[\ref{}]). 

(1) Third Party Cookies: This is the primary method of tracking. Third-party cookies are a type of cookie on a user's browser that are not placed there by the primary website he/she is visiting.
\footnote{This is in contrast with first-party cookies that are placed on a user's browser by the primary website and store important data such as login information and other site specific settings.}.
Such cookies are solely used for tracking users across the web. Hence we identify and remove such cookies. We do so by checking that they are not related to the primary website. 
%making it significantly harder for third-party software to track a user across different websites.

(2) Cache: When a user visits a website, images and other information related to the website is stored on the computer. This can potentially lead to more efficient page loads as website information does not have to be retrieved from the server. However, websites can encode information in such cookies that identifies the user to track the browsing history of a user on that website. This is easily solved by clearing the cache periodically. However as seen from the experimental results, such an intervention is not currently necessary as websites do not tend to forward this information on to advertisers.

(3) Flash Cookies: Such cookies are stored in flash player plugins, such as Adobe Flash Player. Flash cookies are harder to clear without leading to a significantly poorer user experience; specifically, clearing flash cookies (via solely a Google Chrome extension) would require clearing data from every plugin the user has installed. Again as with (2), from the experimental results it is clear that such an intervention is not currently necessary as a minimal number of advertisers go through such a mechanism.

\vspace{2mm}

\noindent \textbf{Overview of User Data Protection Experiment.} We design a simple test to verify whether our system does indeed prevent advertisers from getting access to user data. We do so by clicking on an ad, and counting the number of times that ad is seen again on subsequent websites. We repeat this experiment in three different scenarios: (1) when no cookie clearing is done; (2) when only third-party cookies are blocked; (3) when all types of cookies listed above are blocked. To automate this experiment, we use the software package Selenium to interact with Google Chrome and  Pyautogui to click and perform sequences of keystrokes. We used a combination of the two libraries to iterate through Alexa’s top 100 websites. On each website, our software clicks on every ``iframe" element and uses our ad identification software to classify whether the element is an ad or not
\footnote{Some ads are missed since not all ads are in ``iframes". However this should not bias the results as we miss the same set of ads in all three set of experiments above.}.
If it is an ad, we count whether the ad is the same ad as the one that was initially clicked on the first site visited.

\vspace{2mm}

\noindent \textbf{Result of User Data Protection Experiment.} See Figure \ref{fig:USER_hashing} for results of the above experiment. As desired, we see that when we simply block third-party cookies, we reduce the number of repeat ads show from {\color{red} $14$ to $3$} as compared to if there was no blocking. By blocking all cookies listed above, it does not affect the number of repeat ads seen, indicating that blocking Cache and Flash cookies is currently less important.

\begin{figure}[ht]
\centering
\includegraphics[width=0.7\linewidth]{figures/USER_hashing.png}
\caption{Number of repeated ads seen across 50 websites with different cookie-blocking/hashing schemes.}
\label{fig:USER_hashing}
\end{figure}








==> content/introduction_old.tex <==
\section{Introduction} \label{sec:introduction}
\vspace{-2mm}
\begin{quote} 
\centering 
``\textit{Personal data is the new oil of the internet and the new currency of the digital world }"
\end{quote}
\vspace{-2.2mm}
- Meglena Kuneva, European Consumer Commissioner

\vspace{2mm}

\noindent Over the past two decades, online advertising has become economic backbone of the internet. According to a study by PriceWaterhouseCoopers (PwC) and the Internet Advertising Bureau (IAB), online advertising revenue has grown from USD 100 million in 1996 to USD 88 Billion in 2018, with a 23\% year-on-year growth from 2017 to 2018 (cf.~[\ref{}]). And personal data is one of the key resources advertisers use to show users targeted, relevant ads (cf.~[\ref{}]).

\vspace{2mm}

\noindent \textbf{Inefficiencies in Current System.} However, there still exist two major inefficiencies in the way such data is both bought and sold: (1) from a user's perspective, they do not get to decide what information about themselves is released nor do they get paid for this loss of privacy; (2) from an advertiser's perspective, they have to purchase user data without knowing how much value it is going to provide to them. 

These inefficiencies have led to a swath of societal issues including: (i) increasing ad fraud, where $20-30\%$ of online ad data sold has been deemed to be fraudulent (cf.~[\ref{}]); (ii) an increasing consumer backlash for loss of privacy from unsanctioned data sharing such as in the Facebook-Cambridge Analytica scandal (cf.~[\ref{}]); (iii) an inability to litigate against companies with massive data breaches such as Equifax (cf.~[\ref{}]).

To have a meaningful dialogue about such issues, an important and necessary first step is defining what the ``Value of Data" (VoD) is. However, there do not exist good, real-time pricing mechanisms for data that have been widely adopted. That is why most firms are engaged in inflexible long-term data contracts, rather than paying on a query-by-query basis based on the incremental value the data provides.

\vspace{2mm}

\noindent \textbf{Why Data is a Unique Commodity.} The challenge in designing data pricing systems stems from the nature of data as an asset: (i) user data is freely replicable once sold; (ii) advertisers vary widely and correspondingly, so do their Machine Learning (ML) models; (iii) the usefulness of user data is difficult to verify a priori before running it through a ML model, something which advertisers are not willing to do before purchasing the data. See cf.~[\ref{}] for a more complete overview.

\vspace{2mm}

\noindent \textbf{Our Focus: Click-Through-Rate Estimation.} We focus our efforts on the sale of online user cookie data (e.g. a user's demographic data and browsing history) and the prediction task of estimating user click-through-rate (CTR) for a given ad and user, the key quantity of interest in online advertising (cf.~[\ref{}]). We do so because the sale of online cookie data is one of the large sources of data exchanged (and revenue generated) in modern web-scale systems and the associated network engineering infrastructure is extremely performant with transactions between advertisers and third-party data sellers occurring in less than 200 milliseconds, the time required for a user to load a webpage and for an ad to be served (cf.~[\ref{}]). 

Thus if one can design a feasible solution for this setting, there are many further applications. An important business-to-business example is the sale of potential consumer leads in insurance and mortgage markets using the increasingly adopted Ping-Post Architecture (cf.~[\ref{}]). 

\subsection{Our Contribution}\label{sec:contributions}

We propose a system, Zorro, which aims to address the following aforementioned problems. Our contributions are summarized below.

\vspace{2mm}

\noindent \textbf{System Design.} In Section \ref{sec:system_description} we gave an overview of the key functionalities/modules of Zorro, which are: (1) a principled way to define the VoD; (2) an algorithm to operationalize our definition of the VoD; (3) a module to identify and categorize online ads in an automated fashion; (4) an interface between users, Zorro and advertisers that ensures user data is not inadvertently ``leaked" to advertisers without user permission and that advertisers only pay for user data based on the increased in accuracy it provides to them (in particular, to estimate CTR). 

\vspace{2mm}

\noindent \textbf{Experiments.} In Section \ref{sec:experiments}, we perform four set of experiments to verify the implementation of the modules described above: (1) on a large real-world advertising click dataset, we show we are able to accurately estimate the CTR for a given user and advertiser without access to the advertiser's ML model, the crucial property we require to operationalize our definition of the VoD; (2) on the same click dataset, we show that with respect to our definition of the VoD, there is large variation in the value of each user's data depending on the advertiser's category; (3) we show that we can accurately classify and categorize ads by testing our implementation on popular websites; (4) we show we can indeed prevent user data from being ``leaked" to advertisers by counting the number of repeats ads a user sees depending on whether Zorro is turned ``on" or ``off".

\vspace{2mm}

\noindent \textbf{Forward Looking Intent.} In Section \ref{sec:forward_intent}, we show how one can generalize Zorro, and the associated notion of the VoD to capture forward-looking intent of users. We do so by extending the fundamental data structure of interest, the matrix of (users $\times$ advertisers), to an order-3 tensor of (user-intent $\times$ user $\times$ advertisers).

\subsection{Related Work}\label{sec:related_work}

We divide related work into the three major buckets: (1) real-time online systems to sell user data; (2) data analysis to estimate value of user data; (3) theoretical market mechanisms to sell information.

\vspace{2mm}

\noindent \textbf{Real-Time Systems to Sell User Data.} We compare with two proposed systems that also aim to design real-time pricing mechanisms of online user data in the context of advertising: (i) \{Chaintreau\}; (ii) \{Brave Browser\}. 

\{Chaintreau\}: They propose selling historical user data by posting a price every time a user loads a webpage; whichever advertisers bid above the posted price then acquire user data for that webpage load. User privacy is maintained as a random IP address is generated each time a user loads a webpage. The posted price is then updated for subsequent webpage loads running a standard no-regret update mechanism \textit{per user}. Such a mechanism potentially has limitations. (i) No-regret update schemes are feasible only if user data is relatively static. However, user's browsing patterns are constantly changing and so it is not immediately clear how to adapt a no-regret update scheme to maximize for such a case. (ii) Advertisers either get all of the data and pay the posted price or receive none of it. This could potentially lead to a large loss in revenue. Zorro aims to circumvent these two problems by dividing the transaction into two segments: (i) an offline segment, where each advertiser negotiates a contract with Zorro on how much they value a \textit{marginal increase in accuracy}; (ii) an online segment, where Zorro estimates the marginal increase in accuracy without access to the advertisers ML model (see Section \ref{sec:dsp_zorro_interface} for details of the implementation).

\{Brave Browser\}: They propose a blockchain based system and advocate for a new cryptocurrency named Basic Attention Token (BAT), which allows user to get paid in BAT for viewing ads online. For their system to be widely adopted, it would require an overhaul of the entire, very well-established online advertising ecosystem (see Section \ref{sec:online_ad_market}), which could be challenging as users, advertisers and publishers will all have to buy into this new cryptocurrency. In contrast, Zorro can be plugged into the current ad ecosystem in a straightforward manner. It essentially functions as a novel third-party data seller (i.e. Data Management Platform - see Section \ref{sec:online_ad_market}), which allows users to get paid for providing their data and for advertisers to pay based on the estimated increase in accuracy they experience. Further \{Brave Browser\} does not provide details on how pricing of user data is done, a crucial part of the system.

%Advertisers have to decide on the VoD in real-time based on the raw data provided, a sequence of a user's webpage visits. Given the timespan of a user's webpage load (i.e. 200 milliseconds), this is likely infeasible in practice.

\vspace{2mm}

\noindent \textbf{Data Mining to Estimate Value of User Data.} \textit{DRAFT. Lots of work here. Indicative of how important this problem is. Their focus is data mining large historical datasets to estimate the \underline{average} value of user data per advertiser category. They show that there is indeed value in user data (quote xxx\%), which is encouraging and in line with our work. Zorro is complementary - shows how to operationalize these findings in real-time where advertisers want to estimate VoD on a query-by-query basis.}

\vspace{2mm}

\noindent \textbf{Theoretical Market Mechanisms to Sell Information.} Some well-known works that propose theoretical market designs to sell information include \{Bergemann\}, \{Agarwal\}, \{Acquisti\}. We consider our work to be complimentary to theirs as a fundamental quantity that needs to be estimated in such line of work is the VoD. Zorro proposes a natural, data-driven definition of VoD that can potentially be used to operationalize such systems. Further the works listed have a single buyer and multiple data sellers (e.g. a supply-chain company buying data streams for demand forecasting). This is in contrast with Zorro which is meant for direct, repeated sales of data between multiple buyers and a single seller.


\section{Overview of Real-Time Bidding Ecosystem}\label{sec:online_ad_market}

The Real-Time Bidding (RTB) ecosystem refers to the entire engineering infrastructure associated with buying and selling ads in real-time as users loads webpages. We give a brief summary of the key players in the RTB ecosystem below. Refer to cf.~[\ref{}] for a detailed description of RTB. See Figure \ref{fig:RTB_overview} for a graphical overview (taken from cf.~[\ref{}]). 

\vspace{2mm}

\noindent  \textbf{Advertisers and Demand Side Platforms (DSPs).} Advertisers are companies that want to market their product online. Due to the engineering complexity of the RTB ecosystem, advertisers normally go through a DSP to make bids into the RTB system on their behalf. Thus DSPs essentially serve as algorithmic online advertising agencies. 

For our purposes it is not necessary to differentiate between advertisers and DSPs, and we call the collective entity ``advertisers" for simplicity. 

\vspace{2mm}

\noindent  \textbf{Publishers and Supply Side Platforms (SSPs).} Websites that users visit (e.g. Nytimes, ESPN) are called publishers. When a user loads a publisher webpage, the publisher sends a request out into the RTB system to serve the user ads. Analogous to advertisers, publishers go through SSPs to make requests in the RTB system on their behalf. 
	
\vspace{2mm}

\noindent  \textbf{Ad Exchanges (ADX).} ADX serve as the interface between DSPs and SSPs by matching ad requests from SSPs to bids made by DSPs. They do so by using a combination of first-price and second-price auctions.

\vspace{2mm}

\noindent  \textbf{Data Exchanges a.k.a Data Management Platforms (DMPs).} DMPs serve DSPs, SSPs and ADXs historical user data (usually in real-time) to feed into their models to allow for better, more targeted matchings between users and ads.

\vspace{2mm}

\noindent \textbf{Our Focus is DSP-DMP Interface.} The majority of demand (and source of revenue) for historical user data is due to DSPs. User data is crucial to DSPs as their ML models require such data to make more accurate bids. That is why we focus the discussion of this paper to solve inefficiencies (see Section \ref{sec:introduction} for an overview of the current market inefficiencies) between how Users -- DMPs -- DSPs interface. However as we see in Section \ref{sec:system_description}, none of our system design is specific to the transaction between DSPs and DMPs, and can be extended to include SSPs and ADXs as well.

\begin{figure}
	\centering
	\includegraphics[width=1.0\linewidth,height=4cm]{figures/RTB_overview.png}
	\caption{Key entities in RTB ecosystem.} 
	\label{fig:RTB_overview}
\end{figure}



%\subsection{Motivation}
%\begin{itemize}
%	\item Overview of Online Ad Architecture 
%	\begin{itemize}
%		\item Broad overview
%		\item Double-click on role of DMP's, DSP's
%		\item What data is actually tracked and sold
%	\end{itemize}
%	\item Issues from User’s perspective
%	\begin{itemize}
%		\item Users are not paid for breach of privacy 
%		\begin{itemize}
%		\end{itemize}
%	\end{itemize}
%	\item Issues from DSP’s perspective
%	\begin{itemize}
%		\item Inefficiencies in current data transactions
%		\begin{itemize}
%		\item DSP’s are in long-term contracts with DMP’s. Pay for data without knowing predictive value of it
%		\item Increasing amounts of fraudulent data sold
%		\end{itemize}
%	\end{itemize}
%\end{itemize}

% To simplify, we don't differentiate between DSPs and advertisers








==> content/lit_review.tex <==
\section{Related Work}

\begin{itemize}
\item Augustin Chaintreau 
\item Alessandro Acquisti 
\item Ad Blockers
\item Brave Browser 
\end{itemize}

==> content/system_1.tex <==
\section{Zorro System Overview}\label{sec:system_description}

As mentioned in Section \ref{sec:contributions}, we focus our system design on the following functionalities that are required for Zorro to be feasible in practice:
\begin{enumerate}
	\item \textbf{VoD Definition.} We provide a natural definition of the VoD that captures the incremental value that data provides in estimating CTR. Importantly, our definition does not depend on the ML models of the advertiser. 
%We further justify the use of our definition under a latent variable model (LVM) for the underlying CTR for a given user and advertiser. 
	\item \textbf{VoD Computation.} To operationalize our definition of the VoD, the key requirement is that for a given advertiser, we need to estimate the value of a user's data without access to the advertiser's ML model. We show how one can achieve this using matrix estimation to accurately estimate the CTR in a model agnostic manner.
	\item \textbf{Ad Identification \& Categorization.} A necessary step to do CTR estimation, is to accurately identify when users have clicked on an ad. Further to effectively group advertisers, we need to categorize advertisers in a meaningful and automated way. We show how to do both ad identification and categorization by tying together existing open source software packages.
	\item \textbf{User -- Zorro -- Advertiser Interface.}  We propose an interface/dynamic that ensures advertisers pay for user data based only on the increase in accuracy it brings. And correspondingly, ensures user data is not inadvertently ``leaked" to advertisers without them paying for it. 
\end{enumerate}

In Sections \ref{sec:defining_value_of_data} - \ref{sec:dsp_zorro_interface}, we explain how Zorro performs the above four functions respectively. Our focus will be on ``VoD Definition", ``VoD Computation" and the ``User - Zorro - DSP Interface" as that is where the most significant conceptual contributions are. ``Ad Identification \& Categorization" is a necessary component to make Zorro work and so we will describe how to implement it briefly. Our proposed system design will be corroborated with experiments in Section \ref{sec:experiments}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Defining the Value of Data} \label{sec:defining_value_of_data} 
\subsubsection{Problem Setup - CTR Estimation}
We consider the case where there are $m$ users and $n$ advertisers
\footnote{A ``user" can also refer to a group of users. Similarly, an ``advertiser" can refer to a category of advertisers.}.
For a given user $i$ and advertiser $j$, we define the probability of an ad click as $\text{CTR}_{ij}$. We represent these $m \times n$ CTR quantities for each user, advertiser pair through the (unobserved) matrix $\bM \in [0, 1]^{m \times n}$ where $\bM(i, j) = \text{CTR}_{ij}$.

Unfortunately, we do not get to observe the matrix $\bM$, rather we get sparse, noisy observations of its entries. This is because in reality, most users only see a small percentage of all advertisers; further, for advertisers they do see, they get exposed to their ads only a few times, most likely once. 

We denote our observation matrix as $\bX \in \{[0, 1] \cup \{?\}\}^{m \times n}$. If $\bX_{ij} = ?$, then user $i$ has not been exposed to advertiser $j$. If $\bX_{ij}  \in [0, 1]$, then $\bX_{ij}$ indicates the empirical average of the number of times a user has clicked a particular ad. 

The aim is to infer the CTR for any user $i$ and advertiser $j$ (i.e., $\bM(i, j)$), given only sparse, noisy observations (i.e., $\bX$).

\subsubsection{Latent Variable Model}

For any ML model to effectively learn the underlying CTR given sparse, noisy data, some structure on the matrix $\bM$ must be assumed. A general, flexible way of capturing the underlying structure in social data (e.g. Netflix challenge, product recommendation) is assuming a latent variable model (LVM), arguably the canonical modeling choice in nonparametric regression (cf.~[\ref{}]). 

Specifically for our case, we assume that the CTR for a given user and advertiser is described by the following latent variable model, $\bM(i, j) = f(\theta_i, \omega_j)$ where $f: \Reals^{d_1} \times  \Reals^{d_2} \to [0, 1]$, $\theta_i \in \Reals^{d_1}$ and $\omega_j \in \Reals^{d_2}$. Here $\theta_i, \omega_j$ refer to multi-dimensional variables that denote latent factors associated with user $i$ and advertiser $j$. $f$ is a latent function that maps $\theta_i$ and $\omega_j$ to a value between $0$ and $1$ denoting the underlying CTR for that user, advertiser pair. Note that $f, \theta_i, \omega_j$ are all unobserved (i.e., latent).

\subsubsection{Definition of Value of Data}\label{sec:definition_value_of_data}

Given the LVM described above, we can now provide a definition of the VoD.

\begin{definition}[Value of Data]\label{def:VoD_definition}
For $i \in [m]$ and $j \in [n]$, the value of user $i$'s data to advertiser $j$ is given by,
\begin{equation}
	\VoD = |f(\theta_i, \omega_j) - \Ex_\theta[f(\theta, \omega_j)]|
\end{equation}
where $\Ex_\theta[f(\theta, \omega_j)] = \frac{1}{m} \sum^m_{k = 1} f(\theta_k, \omega_j) $
\end{definition} 

In words, this definition states that the value of user $i$'s data to an advertiser $j$ is the absolute difference between the average CTR for the advertiser across all users (given by $\Ex_\theta[f(\theta, \omega_j)]$) and the CTR for user $i$ (given by $f(\theta_i, \omega_j)$). Though seemingly natural, we consider the definition above as arguably the most important conceptual contribution of this paper and we now make a few remarks regarding it. \\

\vspace{-2mm}

\noindent \textbf{Model Agnostic VoD Definition.} Note that our definition of VoD is not dependent on any particular ML model, but rather just on the prediction task itself (in this case CTR estimation), which is what renders it model agnostic. Further, it is worth noting that we can easily replace CTR with any other quantity of interest in a two-sided market (e.g. likelihood of lead conversion in an auto-insurance marketplace, estimated average spend in a retail marketplace). \\

\vspace{-2mm}

\noindent \textbf{Translation of VoD to a Dollar Amount.} To convert this quantity to a dollar amount, we need to multiply $\VoD$ by how much advertiser $j$ values a marginal increase in accuracy in estimating CTR. For example, it could be be the case that an online healthcare advertiser selling medical drugs values a unit increase in accuracy significantly more than an advertiser selling sports equipment. Hence, the quantity $\VoD$ will need to be scaled to capture this heterogeneity. In Section \ref{sec:dsp_zorro_interface}, we show in detail how such advertiser specific adjustments can be made.  

\subsection{Computing the Value of Data} \label{sec:computing_value_of_data} 

\subsubsection{CTR Estimation via Matrix Estimation}

To make our definition of VoD operational in practice, we need an inference method to estimate CTR without relying on the ML models of the advertisers. This is why we choose matrix estimation, the de facto, non-parametric method to learn the underlying mean of a matrix from sparse, noisy observation. Moreover, it comes with strong theoretical guarantees when a LVM structure is assumed on the underlying mean matrix (cf.~[\ref{}]). Importantly, matrix estimation remains an actively researched area within machine learning with a variety of scalable, production-grade implementations (cf.~[\ref{}]). \\

\vspace{-2mm}

\noindent \textbf{Matrix Estimation Overview.} Matrix estimation is the problem of recovering a data matrix from an incomplete and noisy sampling of its entries. Specifically, there exists an underlying $m \times n$ matrix, $\bM$, of interest. We denote the observation matrix as $\bX$, whose entries are noisy versions of $\bM$, i.e., $\bM(i, j) = \Ex[\bX(i, j)]$. In addition to the observations being noisy, it is further assumed that we only observe a small subset of the entries, i.e., each entry $\bX(i, j)$ is observed with probability $\rho \in [0, 1]$. 

%Common structural assumptions placed on $\bM$ to ensure effective recovery include: (1) $\bM$ is low-rank (cf.~[\ref{}]); (2) $\bM$ can be represented by a latent variable model (cf.~[\ref{}]) (we describe this case in more detail below).

This setup has become of great interest due to its connection to recommendation systems (cf.~[\ref{}]), social network analysis (cf.~[\ref{}]), and graph learning (graphon estimation) (cf.~[\ref{}]). The key realization of this rich literature is that one can estimate the true underlying matrix from noisy, partial observations by simply taking a low-rank approximation of the observed data. We refer an interested reader to recent works such as (cf.~[\ref{}]) and references therein. 

\begin{definition}[Matrix Estimation]\label{def:matrix_estimation}
A matrix estimation algorithm, denoted as $ME : [0, 1]^{m \times n} \to \Reals^{m \times n}$, takes as 
input a noisy matrix $\bX$ and outputs an estimator $\hM$
\end{definition}
 
\vspace{-1mm}

\noindent \textbf{CTR estimation via Matrix Estimation.} CTR estimation can be viewed as a special case of matrix estimation. Specifically, $\bX_{ij}$ can be modeled as the empirical average of a Bernoulli random variable with parameter $f(\theta_i, \omega_j)$. Thus we have that $\frac{1}{\rho} \Ex[\bX_{ij}] = f(\theta_i, \omega_j) = \bM_{ij}$ (recall $\rho$ is the fraction of entries observed). This is exactly the setting in which matrix estimation applies. Thus by applying a standard matrix estimation algorithm, such as Singular Value Thresholding (SVT) (cf.~[\ref{}]), we can reliably infer the underlying $\text{CTR}_{ij}$, simply from sparse, noisy observations (i.e., the small number of click or no click data we have). Refer to Figure \ref{fig:ME_overview} for a graphical depiction of this procedure. Recall again that to carry out this procedure, we do not need access to the advertiser's ML model, simply the click data of any user using the Zorro system. 

\begin{figure*}
	\centering
	\includegraphics[width=0.8\linewidth,height=4cm]{figures/ME_overview.png}
	\caption{Application of matrix estimation to estimate the underlying unobserved CTR, i.e., $\hf(\theta_i, \omega_j)$, from sparse, noisy, $\{0, 1\}$, observations. We assume a latent variable model to capture the underlying CTR structure across users and advertisers; $\theta_i$ and $\omega_j$ are latent factors (e.g. user browsing and purchasing history, advertiser industry category etc.) and $f$ maps these latent factors to the CTR for a user, advertiser pair.} 
	\label{fig:ME_overview}
\end{figure*}

In Section \ref{sec:ME_experiments} we show on a large real-world online advertising datasets, matrix estimation (using Alternating Least Squares) does reliably infer the underlying CTR from partial, noisy click data (after appropriate aggregation of user and advertiser data). We have out-of-sample performance of $R^2 = 0.63$, which is in line with state-of-the-art performance for matrix estimation. \\

\vspace{-2mm}

\noindent \textbf{Estimated Value of Data Definition.} Analogous to Definition \ref{def:VoD_definition}, we define a notion of VoD that can be empirically measured. We recall certain quantities. Let $\bX$ denote the set of sparse noisy observations of user, advertiser data. Let $\hM =  ME(\bX)$ be the estimated underlying CTR after applying matrix estimation on the sparse, noisy observations $\bX$. We denote $\hf(\theta_i, \omega_j) := \hM_{ij}$. 

%There are $m$ users and $n$ advertisers and $\bM \in \Reals^{m \times n}$ denotes the matrix of underlying CTRs (i.e., $\bM_{ij}$ is the underlying CTR for user $i$ and advertiser $j$). Let $f(\theta_i, \omega_j)$ be a latent variable model such that $\bM_{ij} = f(\theta_i, \omega_j)$. 

\begin{definition}[Estimated Value of Data]\label{def:estimated_VoD_definition}
For $i \in [m]$ and $j \in [n]$, the estimated value of user $i$'s data to advertiser $j$ is given by,
\begin{equation}
\hVoD = |\hf(\theta_i, \omega_j) - \Ex_\theta[\hf(\theta, \omega_j)]|
\end{equation}
where $\Ex_\theta[\hf(\theta, \omega_j)] = \frac{1}{m} \sum^m_{k = 1} \hf(\theta_k, \omega_j) $
\end{definition} 

In Section \ref{sec:VoD_experiments}, we show on a large real-world online advertising dataset, user's personal data has value (with respect to Definition \ref{def:estimated_VoD_definition}) ranging from {\color{red} 25\% to 65\%} depending on advertiser category. Importantly, Zorro allows advertiser's to estimate the VoD and hence purchase data on a user-by-user basis, rather than through inefficient long-term contracts as is done now. We provide details in Section \ref{sec:dsp_zorro_interface}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Ad Identification \& Categorization} \label{sec:ad_collection_categorization}
%In this section, we describe how we identify and categorizes ads. Websites do not explicitly state that hyperlinks corresponds to an advertiser (i.e. any external link where the third-party website pays the original website for the redirect) and thus we build an automated ad identification module. Further, accurately classifying the category of an advertiser is a necessary inference task to effectively apply matrix estimation to calculate the VoD.

\subsubsection{Ad Identification}\label{sec:ad_identification}

The focus of this work is banner ads rather than search ads (see cf.~[\ref{}] for details). We do so as the focus of the RTB ecosystem is on banner ads and it is the fastest growing segment of the online advertising market (cf.~[\ref{}]). 

\vspace{2mm}

\noindent \textbf{Definition of Ad.}  Below we describe a straightforward two-level filter system to identify ads when a user clicks on a link on a website. 

\begin{enumerate}
	\item \textbf{Filter Level 1.} We filter for hyperlinks on a website that redirect to a url external to the website itself. 
	\item \textbf{Filter Level 2.} We parse the redirect url to check for substrings that are almost always present when the external link redirects to ads hosted by third-party servers (e.g. AdChoices, Outbrain). We do this by filtering the redirect url using the industry standard Easylist filter list (cf.~[\ref{}]), which is a set of rules designed by AdBlock (cf.~[\ref{}]) to identify ads. 
\end{enumerate}

In Section \ref{sec:ad_experiments}, we show that this simple system effectively identifies whether an external hyperlink is an ad (True Positive and True Negative rate of {\color{red} $83\%$ and $97\%$} respectively). 

\vspace{2mm}

\noindent \textbf{Generalization to Non-Traditional Ads.} It is worth mentioning that companies not traditionally considered advertisers do purchase user data to personalize their website experience for each user (cf.~[\ref{}]). For example, an online marketplace company might purchase user browsing data to decide what products to recommend to that user if he or she comes to their homepage. Again users do not get to choose whether this personal data about them is allowed to be sold nor do they derive income from it. We leave it as future work to generalize our definition of ads (with the necessary adjustments made to the entire Zorro system) to just Filter Level 1.

\subsubsection{Ad Categorization}\label{sec:ad_categorization}

\noindent \textbf{Interactive Advertising Bureau (IAB) Overview.} Ad categorization is an important pre-processing step in grouping advertisers together before performing matrix estimation to compute the VoD. Otherwise, the matrix of users and advertisers (i.e., $\bX$) is too sparse and we cannot effectively infer the underlying CTR for a user, advertiser pair. 
We rely on a widely adopted online advertising taxonomy 
\footnote{``IAB Tech Lab Content Taxonomy Version 2.0"} 
published by the IAB (cf.~[\ref{}]), which advertisers use to serve more relevant content to users. This context taxonomy has four tiers of classification (e.g. ``Style \& Fashion" $\to$ Women's Fashion $\to$ Women's Clothing $\to$	Women's Business Wear). We focus our categorization system on the top two tiers of IAB categories of where there are $28$ and $341$ respectively. 

\vspace{2mm}

\noindent \textbf{Implementing IAB's Categorization.} Given a website, classifying which category it belongs is a challenging task due to the large number of Tier 1 and 2 categories. To automate the process of classifying websites into IAB categories, we input the text within the body of a webpage into a natural language processing software, called uClassify (cf.~[\ref{}]), to classify it to an IAB category.

In Section \ref{sec:ad_experiments}, we show this natural language processing system effectively classifies Wikipedia webpages into the correct IAB category, with an average Tier 1 and Tier 2 accuracy of {\color{red} $67\%$ and $53\%$} respectively. Note that a random guess Tier 1 and Tier 2 guess would have an accuracy of approximately {\color{red} $3.6\%$ and $0.3\%$} respectively.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{User --- Zorro --- Advertiser Interface} \label{sec:dsp_zorro_interface}
In this section, we explain precisely how advertisers will interface with Zorro. Recall this part of the system serves two purposes: (1)
ensure advertisers pay for user data based only on the increase in accuracy it brings; (2) ensure user data is not inadvertently ``leaked" to advertisers without them paying for it. Our approach consists of two steps: (1) an offline step where advertisers negotiate a contract of how much a marginal increase in accuracy is worth to it; (2) an online step where advertisers query Zorro for user data, and they pay for it based on the estimated increase in accuracy they will receive from purchasing it. 

\vspace{2mm}

\noindent \textbf{Offline Contract.} Recall from Section \ref{sec:definition_value_of_data} that each advertiser can have a very different value for an increase in accuracy (consider an online advertiser selling medical drugs vs. sports equipment - how much each values an unit increase CTR can by vastly varying). Thus the estimated VoD (given by Definition \ref{def:estimated_VoD_definition}) needs to be scaled accordingly. Doing this scaling is precisely the purpose of the offline contract between a DSP and Zorro. We describe the contract below.

Recall from Section \ref{sec:ad_categorization} that before doing matrix estimation, we group advertisers together by IAB category (e.g. ``Disease and Conditions", ``Sports Equipment"). Since we estimate the VoD per advertising category, it follows that this offline contract must be defined per IAB category as well. Let there be $C$ such categories. Then for advertiser $j \in [M]$ and category $c \in [C]$, we define a function $p_j^c : [0, 1] \to \Reals^+$. This function, $p_j^c$ summarizes how much advertiser $j$ values an increase in accuracy for category $c$. 
 
For example, a sports equipment advertiser might value a $10\%$ increase in accuracy in the category ``Sports Equipment" to be worth $\$0.1$ while may value a $20\%$ increase in the category ``Disease and Conditions" to only be worth $\$0.001$. The functions $p_j^c$ capture this heterogeneity. Thus a negotiated contract between Zorro and an advertiser $j$ will be the set $P_j := \{p_j^c: \ \text{for} \ c \in [C]\}$

%To gain some intuition, imagine if each $p_j^c$ were a stepwise constant function with a maximum of $L$ steps. Then $P_j$ could be summarized through a matrix, $B \in \Reals^{L \times C}$ where the entry $B_{lc}$ is how much advertiser j values an increase in accuracy in the $l$ to $l+1$th  interval of the function $p_j^c$. \Anish{TO-DO (Add Figure) Refer to Figure $\ref{fig:contract}$ for a graphical overview.}
 
\vspace{2mm}

%{\color{red}  An alternate would be to hold a real-time auction, where only one DSP gets the persons data. But that could be leaving a lot of revenue on the table. Matrix of $\%$ increase in accuracy $\times$ category.} 

\noindent \textbf{Real-Time Interface.} In the example below, let there be $K$ advertisers denoted by $\{\text{AD}_1, \dots, \text{AD}_K\}$ that have negotiated an offline contract with Zorro. We now describe the proposed sequence of interactions that will occur between advertisers and Zorro, each time a user who has the Zorro extension installed loads a publisher's webpage. \Anish{TO-DO (Add Figure): Refer to Figure \ref{fig:overall_architecture} for a graphical overview of entire Zorro system functioning in real-time.} \\

\hrule  
\begin{enumerate} 
	\item A random Zorro IP address is generated and linked with User $i$'s actual IP address. 
	\item User $i$'s with Zorro extension has their webpage request routed through a Zorro proxy server. 
	\item User $i$'s loads a webpage.
	\item The publisher pings a RTB exchange for ad requests and the RTB forwards the requests to advertisers.
%	along with contextual data (e.g. publisher information, contextual data, user Zorro IP Address)
	\item $\{\text{AD}_1, \dots, \text{AD}_K\}$ query Zorro to check if User $i$'s IP address belongs to Zorro \footnote{The random Zorro User IP address could contain a Zorro specific numeric signature to signify that user has the Zorro extension installed}
	\item If User $i$'s IP address belongs to Zorro, then following two actions occur
	\begin{enumerate}
		\item Zorro applies matrix estimation and sends $\{\text{AD}_1, \dots, \text{AD}_K\}$ following two signals: (i) for each $\text{AD}_k$, the estimated VoD of User $i$'s data; (ii) User $i$'s actual personal data (e.g. demographic, interest segments, browsing history).
		\item $\{\text{AD}_1, \dots, \text{AD}_K\}$ pays Zorro based on offline contract defined above. Specifically $\text{AD}_j$ pays,
		 \[\max_{c \in [C]}\bigg(p_j^c\Big(\hVoD\Big)\bigg).\]
	\end{enumerate}
	\item A new random Zorro IP address is generated and linked with User $i$'s actual IP address.
\end{enumerate}
\hrule 

\vspace{4mm}

\noindent \textbf{Why User Data is Not ``Leaked"?} By refreshing a new random Zorro IP address every time a user loads a webpage, we ensure that  to an advertiser who has not negotiated a contract with Zorro, it seems like a random user is loading the webpage. A crucial benefit of this architecture is that user data is never permanently ``leaked" as the random Zorro IP address is constantly refreshed. Thus if a user who has installed Zorro decides to go incognito at some point and no longer receive money for providing their personal data, they easily can.

%\subsubsection{User Interface with Zorro}\label{sec:user_zorro_interface}
%
%\begin{itemize}
%	\item Explanation of chrome extension. What choices user needs to make 
%	\item Mode 1: Zorro totally off
%	\item Mode 2: Zorro prevents all cookie tracking
%	\begin{itemize}
%		\item Describe at a high-level how cooking tracking other than login is prevented
%		\item Describe what permissions user needs to give to allow this
%	\end{itemize}
%	\item Mode 3: Zorro tracks your cookie data and sells it
%	\begin{itemize}
%		\item Explain how Zorro never lets your private identifiable information leave system (see DSP section for details)
%		\item Only features that are predictive leave system
%		\item Allows user to seamlessly move between various modes
%		\item Describe what permissions user needs to give to allow this
%	\end{itemize}
%\end{itemize}


\subsubsection{Model Agnostic Data Contracts}
%A noteworthy benefit of our approach is that for a given advertiser and a particular user, we do not need access to the advertiser's machine learning models to estimate the CTR and in turn the VoD. This is because we can effectively infer the underlying CTR for a user and advertiser by applying matrix estimation, which serves as an effective non-parametric, model agnostic statistical algorithm. Thus we can estimate the VoD for a given user and advertiser, based on just collecting the observed clicks.

The problem of companies not wanting to share their models or their data before a transaction has happened clearly extends far beyond online advertising. This is why so many firms are stuck in inefficient data contracts, where they purchase data based on a long-term agreement or a coarse metric such as the number of API calls they make to a data seller (cf.~[\ref{}]). 

That is why we believe our proposed approach to designing data contracts can serve as a general-purpose, empirically verifiable syxstem for companies to reason about the VoD when sourcing from external vendors. In essence, Zorro can serve as a base to allow data buyers to pay based only on the estimated \textit{increase in accuracy for a clearly defined prediction task}, when purchasing a new dataset from third-parties.

%Data Recommendation System. Empowers less statistically sophisticated advertisers to compete in this market. 

